Assessing User Apprehensions About Mixed Reality Artifacts and Applications: The Mixed Reality Concerns (MRC) Questionnaire

Current research in Mixed Reality (MR) presents a wide range of novel use cases for blending virtual elements with the real world. This yet-to-be-ubiquitous technology challenges how users currently work and interact with digital content. While offering many potential advantages, MR technologies introduce new security, safety, and privacy challenges. Thus, it is relevant to understand users' apprehensions towards MR technologies, ranging from security concerns to social acceptance. To address this challenge, we present the Mixed Reality Concerns (MRC) Questionnaire, designed to assess users' concerns towards MR artifacts and applications systematically. The development followed a structured process considering previous work, expert interviews, iterative refinements, and confirmatory tests to analytically validate the questionnaire. The MRC Questionnaire offers a new method of assessing users' critical opinions to compare and assess novel MR artifacts and applications regarding security, privacy, social implications, and trust.

==> chapters/addendum/original-questions.tex <==
\section{Categorization of Concerns}
\label{sec:categorization}
Four main themes are usual safety, security, privacy + social acceptability. Seams reasonable, but actual explanation for this still missing. 

Items of each theme are based on related work. [...]

For every item, four questions where generated (no further explanation, done by the authors).

Those 4 x 30 questions were sent to experts, they voted on the best question for each item, all other questions were removed.



\subsection{Security}
\todo{Cite "Security and Privacy Approaches in Mixed Reality: A Literature Survey"}
\todo{Explain that sec \& priv properties come from aforementioned publication}

%\begin{table}[h]
%    \centering
    \begin{longtable}{p{14cm}}
        \hline \textbf{Security}\\
        \hline
        \hline \textit{Integrity}\\
        \hline
        SEC-INTEG01: I am concerned about the possibility of unauthorized parties tampering with this MR system, leading to potentially incorrect or even harmful visuals. \\
        SEC-INTEG02: I feel assured that the data and processes within this MR system cannot be modified by anyone without proper authorization. \\
        SEC-INTEG03: I worry that the integrity of this MR system could be compromised, potentially resulting in misleading or harmful content displayed. \\
        SEC-INTEG04: I have confidence in the integrity of the data flow and processing mechanisms within this MR system and feel comfortable using this technology. \\ 
        \hline \textit{Non-Repudiation}\\
        \hline
        SEC-NREP01: I am concerned about the potential for individuals to manipulate or generate false data within the experiences of this MR system and then deny their involvement. \\
        SEC-NREP02: I feel confident that actions performed within this MR system are traceable to their source, preventing involved parties from disowning their actions. \\
        SEC-NREP03: I worry that in scenarios where I use this MR system, the ability to establish the true origin of certain elements might be compromised. \\
        SEC-NREP04: I trust this system in having the means to verify and attribute actions to their responsible parties within MR contexts. \\
        \hline \textit{Availability}\\
        \hline
        SEC-AVAIL01: I am concerned about the possibility of malicious actors disrupting the availability of essential data or processes within this MR system. \\
        SEC-AVAIL02: I feel that uninterrupted access to data and processes within this MR system is available, protecting me from any disruptions that could impact my experience. \\
        SEC-AVAIL03: I worry that external factors could compromise the availability of resources required for the smooth functioning of this MR system. \\
        SEC-AVAIL04: This MR system gives reliable assurance that the availability of necessary elements won't be compromised by external influences. \\
        \hline \textit{Authorization}\\
        \hline
        SEC-AUTHZ01: I am concerned about the potential for unauthorized parties to generate actions or content within the experiences of this MR system, leading to security breaches. \\
        SEC-AUTHZ02: Ensuring that only authorized individuals can initiate actions within this MR system based on their access privileges is clearly taken care of. \\
        SEC-AUTHZ03: I worry that without proper authorization and access control, malicious entities might manipulate or contribute to parts of this MR system in ways that are detrimental. \\
        SEC-AUTHZ04: I'm confident that only approved applications can introduce objects in the environment of this MR system. \\
        \hline \textit{Authentification}\\
        \hline
        SEC-AUTHN01: I am concerned about the possibility of non-authenticated individuals gaining access to this MR system, compromising my privacy and security. \\
        SEC-AUTHN02: I think that this MR system has robust authentication methods in place to ensure that only legitimate individuals can access it. \\
        SEC-AUTHN03: I worry that inadequate authentication mechanisms might allow unauthorized users to access this MR system, potentially leading to misuse or security breaches. \\
        SEC-AUTHN04: I feel assured that only verified and authenticated users can interact with this MR system. \\
        \hline \textit{Identification}\\
        \hline
        SEC-IDENT01: I am concerned about actions within this MR system being performed by unidentified entities, which could potentially compromise security. \\
        SEC-IDENT02: I feel that all parties involved in these MR interactions are clearly identified, establishing accountability and preventing potential security threats. \\
        SEC-IDENT03: With this MR system, I feel that malicious parties could exploit anonymity to engage in harmful actions within MR environments. \\
        SEC-IDENT04: I am sure all actions taken within this MR system are tied to verified identities, maintaining a secure and trustworthy environment. \\
        \hline \textit{Confidentiality}\\
        \hline
        SEC-CONF01: I am concerned about the potential exposure of sensitive or personal data through this MR system to unauthorized parties. \\
        SEC-CONF02: I feel that the confidentiality of sensitive information is maintained and that only authorized parties can access it. \\
        SEC-CONF03: I worry that inadequate measures to safeguard confidential data could lead to privacy breaches and misuse of personal information with this MR system. \\
        SEC-CONF04: I am sure that personal and sensitive data is treated with confidentiality within MR interactions with this system. \\
        \hline
    \end{longtable}
%    \caption{X}
%    \label{table:sec-priv}
%\end{table}

\subsection{Privacy}
\todo{Cite "Security and Privacy Approaches in Mixed Reality: A Literature Survey"}
\todo{Explain that sec \& priv properties come from aforementioned publication}

%\begin{table}[h]
%    \centering
    \begin{longtable}{p{14cm}}
        \hline \textbf{Privacy}\\
        \hline
        \hline \textit{Anonymity \& Pseudonymity}\\
        \hline
        PRIV-ANON01: I am concerned that my personal data on this MR system might be linked back to my specific identity, compromising my privacy. \\
        PRIV-ANON02: I feel that measures have been taken to prevent easy identification on this MR system, maintaining my privacy. \\
        PRIV-ANON03: I worry that a lack of anonymization on this MR system might lead to my personal information being misused. \\
        PRIV-ANON04: I feel assured that my personal data can be dissociated from my identity within this MR system. \\
        \hline \textit{Unlinkability}\\
        \hline
        PRIV-NLINK01: I am concerned about the potential for adversaries to link my identity to my data and interactions within the MR environments of this system, compromising my privacy. \\
        PRIV-NLINK02: Maintaining the unlinkability of my actions and interactions within MR applications from my identity is assured with this system. \\
        PRIV-NLINK03: I worry that a lack of effective unlinkability might allow adversaries to piece together various elements of my MR interactions, potentially revealing sensitive information. \\
        PRIV-NLINK04: I feel assured that my actions and interactions within MR contexts cannot be linked to my identity with this MR system. \\
        \hline \textit{Unobservability \& Undetectability}\\
        \hline
        PRIV-NOBSRV01: I am concerned about the possibility of entities within MR environments on this system being detectable or observable by malicious attackers, potentially compromising my privacy. \\
        PRIV-NOBSRV02: I am sure that entities within MR environments cannot be detected or observed by unauthorized parties on this system. \\
        PRIV-NOBSRV03: I worry that a lack of effective undetectability and unobservability mechanisms might expose my interactions and activities within MR contexts to unwanted surveillance through this system. \\
        PRIV-NOBSRV04: It seems that entities within MR experiences cannot be distinguished from random or latent entities by adversaries. \\
        \hline \textit{Plausible Deniability}\\
        \hline
        PRIV-DENY01: I am concerned about the potential inability to deny my involvement in MR experiences on this system, compromising my privacy. \\
        PRIV-DENY02: Having the option of plausible deniability within MR contexts is important to protect my privacy and control over the information I generate or interact with. \\
        PRIV-DENY03: I worry using this MR system might lead to unintended disclosure of my actions or interactions within MR environments. \\
        PRIV-DENY04:  I can maintain plausible deniability regarding my actions and interactions within this MR system. \\
        \hline \textit{Content Awareness}\\
        \hline
        PRIV-AWARE01: I am concerned about the possibility that sensitive data might be captured and utilized without my awareness, compromising my privacy on this MR system. \\
        PRIV-AWARE02: I know the data flows and processes that MR applications on this system use, especially for sensitive information. \\
        PRIV-AWARE03: I worry that a lack of transparency in how MR applications handle and process data might lead to unintended disclosures of personal information on this MR system. \\
        PRIV-AWARE04: I am not aware of what data is being captured and utilized by this MR system. \\
        \hline \textit{Policy \& Consent Compliance}\\
        \hline
        PRIV-COMPL01: I am concerned about the potential of this MR system to disregard privacy and security policies, putting my personal information at risk. \\
        PRIV-COMPL02: I am sure that this MR system adheres to established privacy and security policies. \\
        PRIV-COMPL03: I worry that inadequate policy compliance by third-party applications or services could lead to potential violations of my privacy or security with this MR system. \\
        PRIV-COMPL04: I do not feel like this MR system adheres to common privacy and security policies. \\
        \hline
    \end{longtable}
%    \caption{X}
%    \label{table:sec-priv}
%\end{table}

\subsection{Safety}
\todo{Cite "The Ethics of Realism in Virtual and Augmented Reality"}
\todo{Explain that categories come from aforementioned publication (implications)}

%\begin{table}[h]
%    \centering
    \begin{longtable}{p{14cm}}
        \hline \textbf{Safety}\\
        \hline
        \hline \textit{Social Isolation}\\
        \hline
        SAF-ISO01: I am concerned that increased usage of this MR system could lead to reduced face-to-face interactions, potentially causing social isolation. \\
        SAF-ISO02: If this MR system becomes as prevalent as current mobile devices, I worry that it might negatively impact my ability to engage in real-life social interactions. \\
        SAF-ISO03: I feel that this MR system could lead to me limiting my interactions with others in physical environments, leading to feelings of isolation. \\
        SAF-ISO04: I think that this MR system would be detrimental for many people, as excessive usage might result in social isolation. \\
        \hline \textit{Preference for Virtual Social Interactions}\\
        \hline
        SAF-PREF01: I am concerned that widespread use of this MR system could lead to a preference for virtual social interactions over real-life interactions. \\
        SAF-PREF02: I worry that due to this MR system, people might withdraw from physical society, impacting mental health and social norms. \\
        SAF-PREF03: I am cautious about the potential for MR experiences on this system to become so captivating that they overshadow face-to-face interactions, leading to a shift in societal norms. \\
        SAF-PREF04: I am concerned about the potential negative effects of preferring virtual social interactions with this MR system. \\
        \hline \textit{Body Neglect}\\
        \hline
        SAF-BODY01: I am concerned that this MR system's immersive nature could lead to neglecting my physical well-being and daily responsibilities. \\
        SAF-BODY02: I worry that I might inadvertently neglect my own health and responsibilities in favor of virtual interactions with this MR system. \\
        SAF-BODY03: I am feeling cautious about the possibility of getting so engrossed in MR activities on this system that I overlook important aspects of my physical health and personal commitments. \\
        SAF-BODY04: The MR experiences with this system are so captivating that I worry that people might prioritize virtual activities over their health and important life obligations. \\
        \hline \textit{Imitative Behavior}\\
        \hline
        SAF-IMIT01: I am concerned that the immersive nature of MR experiences on this system might encourage behaviors that I would not engage in outside of the virtual environment. \\
        SAF-IMIT02: Using this MR system, I worry about the potential for negative impacts on my behavior outside of the virtual world. \\
        SAF-IMIT03: I am cautious about the possibility that engaging in certain behaviors within MR environments of this system might lead to a greater likelihood of engaging in similar behaviors in real life. \\
        SAF-IMIT04: I fear that with this MR system, it becomes increasingly hard to maintain a clear distinction between virtual behavior and real-life behavior. \\
        \hline \textit{Persuasion}\\
        \hline
        SAF-PERS01: I am concerned about the potential of this MR system to influence my emotions and behaviors in ways that could be detrimental to my well-being. \\
        SAF-PERS02: The persuasive nature of MR experiences on this MR system, worries me because they might change my perceptions and behaviors without my conscious choice. \\
        SAF-PERS03: I am cautious about the ethical implications of using this MR system, as it might intentionally influence emotions or behaviors for negative purposes. \\
        SAF-PERS04: I do not have a clear understanding of how this MR system might attempt to persuade and influence me. \\      
        \hline \textit{Unexpected Horror}\\
        \hline
        SAF-HOR01: I am concerned that engaging with this MR system might expose me to unexpected and distressing horror content that could negatively impact my mental well-being. \\
        SAF-HOR02: The possibility of encountering unexpected horror content within MR environments of this system worries me. \\
        SAF-HOR03: I am cautious about the potential for MR experiences with this system to include horrors that I did not anticipate or consent to. \\
        SAF-HOR04: I feel unsure about using this MR system, as I could experience realistic horror scenarios that I do not want to be part of. \\
        \hline \textit{Pornography and Exposure to Violence}\\
        \hline
        SAF-EXPO01: I am concerned about the potential exposure to explicit and violent content with this MR system, as the realism and first-person perspective might have societal consequences. \\
        SAF-EXPO02: The possibility of encountering explicit or violent scenes with this MR system worries me, as the immersive nature of these experiences could impact how I perceive such content. \\
        SAF-EXPO03: I am cautious about the effects of experiencing realistic explicit or violent content within MR environments on this system. \\
        SAF-EXPO04: I feel that the MR experiences with this system are so realistic, that the consumation of explicit or violent content could have a lasting impact on my well-being. \\
        \hline \textit{Extreme Violence and Assault}\\
        \hline
        SAF-EXTR01: I fear that the depiction of extreme acts of violence and assault in MR experiences with this system could potentially desensitize individuals to these behaviors. \\
        SAF-EXTR02: I am concerned that the inclusion of explicit and violent content involving virtual characters in MR experiences on this system might blur the line between fantasy and reality, possibly impacting how individuals perceive and respond to such actions in real life. \\
        SAF-EXTR03: I believe that MR experiences on this system featuring extreme violence and assault raise serious ethical questions, as they could contribute to normalizing these behaviors by portraying them in a virtual context. \\
        SAF-EXTR04: I think that the realistic portrayal of extreme physical and sexual assault with this MR system may trigger aggressive tendencies in me. \\
        \hline \textit{Lack of Common Environments}\\
        \hline
        SAF-ENVIR01: I am concerned that the use of this MR system might lead to a fragmentation of shared societal norms and values, as personalized environments could result in people having drastically different experiences and perceptions of reality. \\
        SAF-ENVIR02: I believe that with this MR system, the lack of visibility into other individuals' MR environments could hinder meaningful public discussions about social and political issues. \\
        SAF-ENVIR03: I fear that the MR environments of this system could lead to the potential loss of a common sense of reality and shared experiences. \\
        SAF-ENVIR04: I am apprehensive about the idea that prolonged use of this MR system might diminish the concept of a 'public sphere'. \\
        \hline \textit{Lack of Ground Truth}\\
        \hline
        SAF-TRUTH01: I am concerned that the persuasive power of this MR system to create convincing sensory experiences might lead to situations where people believe these experiences to be true, even though they might be manipulated or altered by those controlling the technology. \\
        SAF-TRUTH02: I believe that the potential of this MR system to manipulate sensory experiences could lead to challenges in legal and factual matters, as people may have difficulty distinguishing between genuine experiences and artificially generated ones. \\
        SAF-TRUTH03: The capacity of this MR system to decouple sensory experiences from ground truth makes me uneasy about the potential erosion of trust in shared reality. \\
        SAF-TRUTH04: I am apprehensive about the implications of using this MR system, as it has the potential to undermine the reliability of sensory experiences as a basis for truth and reality, which could have far-reaching consequences for social cohesion and understanding. \\
        \hline \textit{Persuasive Advertising}\\
        \hline
        SAF-ADS01: I am concerned about the potential intrusion of persuasive advertising in MR experiences on this system. \\
        SAF-ADS02: I believe that the immersive nature of this MR system could make persuasive advertising more impactful and difficult to ignore. \\
        SAF-ADS03: The idea of being continuously exposed to advertising with this MR system, without clear indicators that I am being persuaded, makes me uneasy about the potential manipulation of my preferences and choices. \\
        SAF-ADS04: I am apprehensive about the possibility of having no way to avoid advertising with this MR system, as this could limit my freedom to engage with the technology without constant commercial influence. \\
        \hline
    \end{longtable}
%    \caption{X}
%    \label{table:saf}
%\end{table}

\subsection{Social Acceptance}
\todo{Explain that the following determinants are, in part, taken from "Socio-psychological determinants of public acceptance of technologies: A review". The ten determinants that were most used are: Perceived risk, perceived benefit, trust and culpability, knowledge, individual differences, and attitude. In the following, only fitting ones were chosen and some were added (reasoning?).}

%\begin{table}[h]
%    \centering
    \begin{longtable}{p{14cm}}
        \hline \textbf{Social Acceptance}\\
        \hline
        \hline \textit{Perceived Health Implications}\\
        \hline
        ACC-HLTH01: I am concerned that the prolonged use of this MR system will be seen as unhealthy. \\
        ACC-HLTH02: I am apprehensive that using this MR system might raise health-related questions from others, potentially making me feel self-conscious about the technology's impact on my well-being.\\
        ACC-HLTH03: I worry about the potential stigma attached to using this MR system due to health concerns. \\
        ACC-HLTH04: I'm worried about the health-related assumptions others might make about me using this MR system. \\
        \hline \textit{Social Outcast}\\
        \hline
        ACC-OUTC01: I am concerned that using this MR system might make me appear socially isolated or disconnected from others in my physical environment. \\
        ACC-OUTC02: I'm concerned that wearing this MR system might raise questions about my priorities and lifestyle choices. \\
        ACC-OUTC03: I have reservations about how others might perceive me when using this MR system, as it could lead to assumptions about my willingness to prioritize virtual experiences over real-world social interactions and activities. \\
        ACC-OUTC04: I'm concerned that using this MR device might make others view me as detached from reality. \\
        \hline \textit{Interactions}\\
        \hline
        ACC-IACT01: I worry that the use of this MR system could lead to misunderstandings or misinterpretations in my interactions with people around me, affecting the quality of my social interactions. \\
        ACC-IACT02: I worry that using this MR system could lead to social awkwardness or discomfort in group settings. \\
        ACC-IACT03: I'm unsure if using this MR system in public could affect how others perceive my social skills. \\
        ACC-IACT04: I have reservations about how this MR system might influence my interactions with others. \\
        \hline \textit{Trust}\\
        \hline
        ACC-TRST01: I worry that using this MR system might lead others to question my credibility and reliability. \\
        ACC-TRST02: I am concerned that people might view me differently or doubt my intentions when I use this MR system. \\
        ACC-TRST03: I feel uneasy about the potential impact of this MR system on how others perceive my authenticity and trustworthiness. \\
        ACC-TRST04: I have reservations about the level of trust others will have in me as a user of this MR technology, which could affect my relationships. \\
        \hline \textit{Family \& Friends}\\
        \hline
        ACC-FAM01: I feel unsure about how my friends and family might react to me using this MR technology. \\
        ACC-FAM02: I have concerns that my loved ones might not fully understand or support my choice to engage with this MR system. \\
        ACC-FAM03: I feel uncertain about how my friends and family will react to me incorporating this MR device into my daily life. \\
        ACC-FAM04: I am hesitant about potential differences in opinions between me and my friends or family regarding the appropriateness of using this MR system. \\
        \hline \textit{Perceived Risk}\\
        \hline
        ACC-RSK01: I have concerns that some people may consider using this MR system to be a reckless choice. \\
        ACC-RSK02: I feel unsure about how others might perceive the level of risk associated with me using this MR device. \\
        ACC-RSK03: I'm hesitant about potential negative judgments from others who might find my engagement with this MR technology to be too adventurous. \\
        ACC-RSK04: I'm worried that others might view my use of this MR technology as too risky or daring. \\
        \hline
    \end{longtable}
%    \caption{X}
%    \label{table:acc}
%\end{table}

==> chapters/focus-group-one.tex <==
\section{First Focus Group}
\label{sec:focusgroup1}

\todo{Results of student work}
